A phenomenological connectivity measure for the pore space of rocks

The interconnectivity of the porous space is an important characteristic in the study of porous media and their transport properties. Hence we propose a way to quantify it and relate it with the intrinsic permeability of rocks. We propose a measure of connectivity based on geometric and topological information of pore-throat network, which are models built from microtomographic images, and we obtain an analytical method to compute that property. The method is expanded to handle rocks that present a higher degree of heterogenity in the porous space, which characterization requires images from different resolutions (multiscale analysis). Trying to expand the methodology beyond the scope of images, we also propose a new interpretation for the experiment that generates the mercury intrusion curve and calculate the permeability. The methodology was applied to images of 11 rocks, 3 sandstone and 8 carbonate rock samples, and to the experimental mercury intrusion curve of 4 tight gas sand rock samples. We observe as result the existence of a correlation between the experimental and the predicted values. The notions of connectivity developed in this work seek above all to characterize a porous material before a typical macroscopic phenomenology.

==> bibitem.tex <==
%
% Bibliografia em bibitems
%

\newcommand{\etal}{\textit{et al.}}
\newcommand{\cidade}{\textcolor{IndianRed3}{***}}
% \newcommand{\alertaBib}[1]{\textcolor{IndianRed3}{\footnotesize*ALERTA: #1*}}
\newcommand{\alertaBib}[1]{\textcolor{black}{\itshape\footnotesize*#1*}}

\begin{thebibliography}{99}

\bibitem{Scheidegger1963}
A. E. Scheidegger,
in \emph{Handbuch der Physik}
(Springer-Verlag, Berlim, 1963).

\bibitem{Dullien1979}
F. Dullien,
\emph{Porous Media}
(Academic Press, San Diego, 1979).

\bibitem{Fatt1956a}
I. Fatt,
Petrol. Transactions AIME \textbf{207}, 144 (1956).

\bibitem{Fatt1956b}
I. Fatt,
Petrol. Transactions AIME \textbf{207}, 160 (1956).

\bibitem{Fatt1956c}
I. Fatt,
Petrol. Transactions AIME \textbf{207}, 164 (1956).

\bibitem{ChatzisDullien1977}
I. Chatzis e F. Dullien,
J. Can. Pet. Technol. \textbf{16}, 97 (1977).

\bibitem{VanMarcke2010}
P. Van Marcke \etal,
Transport in Porous Med. \textbf{85}, 451 (2010).

\bibitem{Okabe2005}
H. Okabe M. Blunt,
J. Petrol. Sci. Eng. \textbf{46}, 121 (2005).

\bibitem{Fernandes1996}
C. P. Fernandes \etal,
Phys. Rev. E \textbf{54}, 1735 (1996).

\bibitem{Vinegar1987}
H. J. Vinegar e S. L. Wellington,
Rev. Sci. Instrum \textbf{58}, 96 (1987).

\bibitem{Dunsmuir1991}
J. H. Dunsmuir \etal,
em \emph{Proceedings of 66th SPE Conference},
Dallas, TX, n. SPE 22860 (1991).

\bibitem{BryantBlunt1992}
S. Bryant e M. Blunt,
Phys. Rev. A \textbf{46}, 2004 (1992).

\bibitem{Landisa2010}
E. N. Landisa e D. T. Keaneb,
Mater. Charact. \textbf{61}, 1035 (2010).

% \bibitem{VanMarcke2010}
% P. Van Marcke \etal,
% Transport in Porous Med. \textbf{85}, 451 (2010).

% \bibitem{AlKharusi2007Tese}
% A. S. Al Kharusi,
% \emph{Pore-scale characterization of carbonate rocks}
% (Imperial College London, Londres, 2007).

\bibitem{AlKharusi2007}
A. S. Al Kharusi e M. J. Blunt,
J. Petrol. Sci. Eng. \textbf{56}, 219 (2007).

\bibitem{HuDongPRE2009}
H. Dong e M. Blunt,
Phys. Rev. E \textbf{80}, 1 (2009).

\bibitem{Cunha2013Physicae}
A. R. Cunha,
\emph{Caracterização de sistemas porosos de rochas reservatório de petróleo a partir da extração de redes poro-ligações}
(DM, UFSC, Florianópolis, 2012).
% % A. R. Cunha \etal,
% % \alertaBib{Submetido à Physic\ae{}}
% \alertaBib{referência provisória}
% % Consta na Dissertação de Mestrado do autor (Artigo submetido).
% Obra do autor.

\bibitem{Cunha2012M}
A. R. Cunha,
\emph{Caracterização de sistemas porosos de rochas reservatório de petróleo a partir da extração de redes poro-ligações}
(DM, UFSC, Florianópolis, 2012).
% \alertaBib{referência provisória}
% % Dissertação de Mestrado do autor.
% Obra do autor.

\bibitem{BemSilva2012M}
A. F. B. Silva,
\emph{Caracterização do espaço poroso em rochas por esferas máximas exatas}
(DM, UFSC, Florianópolis, 2012).
% \alertaBib{referência provisória}
% % Dissertação de Mestrado de colaborador 1.
% Obra de colaborador.

\bibitem{JefersonRamos2012M}
J. V. Ramos,
\emph{Validação do cálculo de dados petrofísicos com base na caracterização de rochas de reservatório}
(DM, UFSC, Florianópolis, 2012).
% \alertaBib{referência provisória}
% % Dissertação de Mestrado de colaborador 2.
% Obra de colaborador.

\bibitem{Kay2005}
S. Kay,
\emph{Intuitive Probability and Random Processes using Matlab$^{\tiny®}$}
(Springer, Nova Iorque, 2005).

\bibitem{Nutting1930}
P. G. Nutting,
Am. Assoc. Petr. Geol. B. \textbf{14}, 1337 (1930).

\bibitem{Russ2011}
J. C. Russ,
\emph{The image processing handbook}
(CRC Press, Boca Raton, 6ª ed., 2011).

\bibitem{Sun2012}
T. Sun \etal,
Int. J. of Oil, Gas and Coal Technology \textbf{5}, 249 (2012).

\bibitem{Mariam2010}
M. I. Al-Marzouqi \etal,
Oilfield Review \textbf{22}, 40 (2010). 

\bibitem{Graham2012}
I. G. Graham \etal, eds.,
Numerical Analysis of Multiscale Problems
(Springer, Berlim, 2012)

\bibitem{Tsakiroglou2012}
C. D. Tsakiroglou,
Transport in Porous Med. \textbf{94}, 525 (2012).

% \bibitem{Ichikawa2012}
% Y. Ichikawa e A. P. S. Selvadurai,
% Transport Phenomena in Porous Media: Aspects of Micro/Macro Behaviour
% (Springer, Heidelberg, 2012)

\bibitem{Tiab2004}
D. Tiab e E. C. Donaldson,
\emph{Petrophysics}
(Gulf Professional Publishing, Oxford, 2004).

\bibitem{Glover2010}
P. W. J. Glover,
Geophysics \textbf{76}, E247 (2010).

\bibitem{Montaron2009}
B. Montaron, B.
Petrophysics \textbf{50}, 102 (2009).

\end{thebibliography}

